A Dimensionality Reduction Approach for Convolutional Neural Networks

The focus of this paper is the application of classical model order reduction techniques, such as Active Subspaces and Proper Orthogonal Decomposition, to Deep Neural Networks. We propose a generic methodology to reduce the number of layers of a pre-trained network by combining the aforementioned techniques for dimensionality reduction with input-output mappings, such as Polynomial Chaos Expansion and Feedforward Neural Networks. The necessity of compressing the architecture of an existing Convolutional Neural Network is motivated by its application in embedded systems with specific storage constraints. Our experiment shows that the reduced nets obtained can achieve a level of accuracy similar to the original Convolutional Neural Network under examination, while saving in memory allocation.

==> sections/preamble.tex <==
%\usepackage{subfig}
\usepackage{subcaption}
\usepackage{pgfplots}
\usepackage{pgfplotstable}
\usepgfplotslibrary{groupplots}
\usepgfplotslibrary{fillbetween}
\usepackage{mathtools}
\usepackage{multicol}
\usepackage{comment}
\usepackage{booktabs}
\pgfplotsset{compat=1.5}
\usepackage{amssymb}
\usepackage{url}
\usepackage{bm}
\usepackage{algorithm}
%\usepackage{algorithmic}
\usepackage{algpseudocode}
%\usepackage[doublespacing]{setspace}
\usepackage{multirow}


\usepackage{pdfsync}

\usepackage{float}
\usepackage{tabularx}
\usepackage{enumerate}
\usepackage{array}
\usepackage{xspace}
\usepackage{tikz}
\usepackage{tikzsymbols}
\usetikzlibrary{calc,trees,positioning,arrows,chains,shapes.geometric,%
    decorations.pathreplacing,decorations.pathmorphing,shapes,%
    matrix,shapes.symbols, decorations.markings, patterns,fit,quotes,%
    arrows.meta}

\usepackage{authblk}

\usepackage{hyperref}
\usepackage[draft,inline,marginclue]{fixme}
% add yours
\FXRegisterAuthor{mt}{amt}{MT}
\newcommand{\MT}[1]{\mtwarning{#1}}

\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{corol}{Corollary}

\newcommand{\TODO}[1]{{\color{red}#1}}
\newcommand{\mupar}{\ensuremath{\boldsymbol{\mu}}}
\newcommand{\etapar}{\ensuremath{\boldsymbol{\eta}}}
\newcommand{\R}{\ensuremath{\mathbb{R}}}
\newcommand{\x}{\ensuremath{\mathbf{x}}}
\newcommand{\z}{\ensuremath{\mathbf{z}}}
\newcommand{\y}{\ensuremath{\mathbf{y}}}
\newcommand{\cpar}{\ensuremath{\mathbf{c}}}
\newcommand{\fulldim}{\ensuremath{\mathcal{N}}}
\newcommand{\reddim}{\ensuremath{N}}
\newcommand{\pardim}{\ensuremath{m}}

\newcommand{\fullspace}{\ensuremath{\mathbb{X}^\fulldim}}
\newcommand{\redspace}{\ensuremath{\mathbb{X}^\fulldim_\reddim}}
\newcommand{\parspace}{\ensuremath{{\bf P}}}
\newcommand{\Xtrain}{\ensuremath{\mathbf{X}}}
\newcommand{\Xtest}{\ensuremath{\mathbf{\Bar{X}}}}
\newcommand{\ytrain}{\ensuremath{\mathbf{y}}}
\newcommand{\ytest}{\ensuremath{\mathbf{\Bar{y}}}}
\newcommand{\V}{\ensuremath{\mathbf{V}}}
\newcommand{\Spar}{\ensuremath{\mathbf{S}}}
\newcommand{\Cpar}{\ensuremath{\mathbf{C}}}
\newcommand{\Gpar}{\ensuremath{\mathbf{G}}}
\newcommand{\Sigmapar}{\ensuremath{\mathbf{\Sigma}}}
\newcommand{\U}{\ensuremath{\mathbf{U}}}
\newcommand{\diag}{\text{diag}}
\newcommand{\Lambdapar}{\ensuremath{\boldsymbol{\Lambda}}}
\newcommand{\phipar}{\ensuremath{\boldsymbol{\phi}}}
\newcommand{\Phipar}{\ensuremath{\boldsymbol{\Phi}}}
\newcommand{\alphapar}{\ensuremath{\boldsymbol{\alpha}}}
\newcommand{\thetapar}{\ensuremath{\boldsymbol{\theta}}}








